TrTr: Visual Tracking with Transformer

Template-based discriminative trackers are currently the dominant tracking methods due to their robustness and accuracy, and the Siamese-network-based methods that depend on cross-correlation operation between features extracted from template and search images show the state-of-the-art tracking performance. However, general cross-correlation operation can only obtain relationship between local patches in two feature maps. In this paper, we propose a novel tracker network based on a powerful attention mechanism called Transformer encoder-decoder architecture to gain global and rich contextual interdependencies. In this new architecture, features of the template image is processed by a self-attention module in the encoder part to learn strong context information, which is then sent to the decoder part to compute cross-attention with the search image features processed by another self-attention module. In addition, we design the classification and regression heads using the output of Transformer to localize target based on shape-agnostic anchor. We extensively evaluate our tracker TrTr, on VOT2018, VOT2019, OTB-100, UAV, NfS, TrackingNet, and LaSOT benchmarks and our method performs favorably against state-of-the-art algorithms. Training code and pretrained models are available at https://github.com/tongtybj/TrTr.

==> Makefile <==
# Makefile tips: http://www.ie.u-ryukyu.ac.jp/~e085739/c.makefile.tuts.html

LATEX=platex
MAKEINDEX=makeindex
BIBTEX=pbibtex
LABPAT="^LaTeX Warning: Label(s) may have changed\."
FIGDIR = figs

PDFOPEN = gnome-open

THISDIR = 2021_ICCV
BASE1=main
CLS=ieeetran.cls
SRCS=main.tex

bases = $(BASE1)
targets = $(bases:%=%.pdf) # http://www.ne.jp/asahi/hishidama/home/tech/unix/cmd/make2.html
bbls = $(bases:%=%.bbl)
#$(warning bbls = $(bbls))

.SUFFIXES: .txt .tex .bbl .bb .jpg .JPG .png .PNG .bmp .BMP .pdf

.jpg.bb:
	@(ebb -b $< 2>/dev/null;)

.JPG.bb:
	@(ebb -b $< 2>/dev/null;)

.png.bb:
	@(ebb -b $< 2>/dev/null;)

.PNG.bb:
	@(ebb -b $< 2>/dev/null;)

.pdf.bb:
	@(ebb -b $< 2>/dev/null;)

BB_FILES = $(shell find ${FIGDIR} -name "*.jpg" | sed s/jpg/bb/g)
BB_FILES += $(shell find ${FIGDIR} -name "*.JPG" | sed s/JPG/bb/g)
BB_FILES += $(shell find ${FIGDIR} -name "*.png" | sed s/png/bb/g)
BB_FILES += $(shell find ${FIGDIR} -name "*.PNG"| sed s/PNG/bb/g)
BB_FILES += $(shell find ${FIGDIR} -name "*.pdf"| sed s/pdf/bb/g)

#$(warning BB_FILES = $(BB_FILES))

%.pdf: %.dvi
	dvipdfmx -V 6 -p letter $<

%.dvi: %.tex
	$(LATEX) $*
	while grep $(LABPAT) $*.log; do $(LATEX) $<; done

%.bbl: %.bib
	$(LATEX) $*
	$(BIBTEX) $*
	$(LATEX) $*

.PHONY: all clean

all: clean $(targets)

bb: $(BB_FILES)

$(BASE1).dvi: bb $(BASE1).bbl $(SRCS)

#$(bbls): $(CLS)

clean:	bb_bib_clean
	rm -rf *~ *.log *.dvi *.pdf *.aux *.bbl *.blg *.toc *.flc *.bak *.bmc fig.pbm

bb_bib_clean:
	rm -f $(FIGDIR)/*.bb $(FIGDIR)/*/*.bb
	(cd $(FIGDIR); rm -f *~; rm -f *#)

open:
	${PDFOPEN} $(bases).pdf

